Ubic: Bridging the gap between digital cryptography and the physical world

Advances in computing technology increasingly blur the boundary between the digital domain and the physical world. Although the research community has developed a large number of cryptographic primitives and has demonstrated their usability in all-digital communication, many of them have not yet made their way into the real world due to usability aspects. We aim to make another step towards a tighter integration of digital cryptography into real world interactions. We describe Ubic, a framework that allows users to bridge the gap between digital cryptography and the physical world. Ubic relies on head-mounted displays, like Google Glass, resource-friendly computer vision techniques as well as mathematically sound cryptographic primitives to provide users with better security and privacy guarantees. The framework covers key cryptographic primitives, such as secure identification, document verification using a novel secure physical document format, as well as content hiding. To make a contribution of practical value, we focused on making Ubic as simple, easily deployable, and user friendly as possible.

==> sections/11evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}

To investigate the feasibility of using QR codes within our document format, we first performed an evaluation of the scanning times for different codes as defined by the QR code standard. Specifically, we compared V1 (21x21 pixels), V2 (25x25 pixels), V3 (29x29 pixels), V4 (33x33 pixels), V10 (57x57 pixels) and V40 (177x177 pixels). We generated QR codes for each of these sizes and scanned each code 20 times using a custom app running on GoogleGlass. Scans were performed in a normal office environment at typical usage distances of about xx cm and with varying viewpoints.

As can be seen from Figure \ref{fig:scanning_time}, the scanning time increases steadily the larger the QR code. While scanning times for V1-4 was below 1 second, scanning of V10 type codes already took more than 15 seconds. V40 codes are impractical to use for our purposes given that the scanning time for such codes increases to nearly one minute.

\begin{figure}[hbt]
\centering
  \includegraphics[width=7cm]{figures/scanning_time}
  \caption{Scanning time for different QR codes in seconds average over 20 scans. Scans were performed at typical usage distances and from  different viewpoints.}\label{fig:scanning_time}
\end{figure}

%\msimkin{
%    Evaluation and comparison of the computer vision techniques with common things like QR-Codes and so on. 
%    What could be a good measurement for how good \SeVi actually works in practice? At least we should 
%    describe how well it is usable in the real world.
%}

